Event Ticket Price Prediction with Deep Neural Network on Spatial-Temporal Sparse Data

Event ticket price prediction is important to marketing strategy for any sports team or musical ensemble. An accurate prediction model can help the marketing team to make promotion plan more effectively and efficiently. However, given all the historical transaction records, it is challenging to predict the sale price of the remaining seats at any future timestamp, not only because that the sale price is relevant to a lot of features (seat locations, date-to-event of the transaction, event date, team performance, etc.), but also because of the temporal and spatial sparsity in the dataset. For a game/concert, the ticket selling price of one seat is only observable once at the time of sale. Furthermore, some seats may not even be purchased (therefore no record available). In fact, data sparsity is commonly encountered in many prediction problems. Here, we propose a bi-level optimizing deep neural network to address the curse of spatio-temporal sparsity. Specifically, we introduce coarsening and refining layers, and design a bi-level loss function to integrate different level of loss for better prediction accuracy. Our model can discover the interrelations among ticket sale price, seat locations, selling time, event information, etc. Experiments show that our proposed model outperforms other benchmark methods in real-world ticket selling price prediction.

==> Prelim.tex <==

% \section{Preliminaries}
% \label{sec:prelim}
% In this section, we mathematically define our problem setting. We start off by formally defining our notation. 
% \subsection{Problem Definition}
% Given the selling records (price of all the sold tickets and the corresponding seat locations) and other relevant information of multiple past events, we want to predict the price of the coming event at a particular time. 
% We denote $p_{t_j}^{(r,c)}$ as the ticket price of the seat in $r$-th row $c$-th column at time $t_j$. Our goal is to design a model $F$ to predict 
% \begin{align}
% \label{eq:goal}
% & p_{t_{j+1}}^{(r,c)} = F(P_{1},...P_{t_j}, C_{1},...C_{t_j}),  
% \end{align}  
% where $P_{t_j}$ are the available selling price for all the seats at time $t_j$, and $C_{t_j}$ are the corresponding context features (event date, weather, team stars etc.) at time $t_j$. 

% Due to data sparsity by nature, $p_{t_{j}}^{(r,c)}$ is very likely to be empty because the seat is not sold at time $t_j$. In other words, $P_{t_j}$ is very sparse, which makes traditional regression methods inapplicable. To solve this problem, we propose a coarsening layer on both temporal and spatial dimensions as follows. 

% \subsection{Coarsening Layer}
% First of all, we define the set of non-overlapping blocks $K = \{k_1,k_2,...,k_n\}$ as block-wise partitions of a court, and the set of non-overlapping time intervals as $T = \{t_1,t_2,...t_m\}$. 
% Each block $k_i$ consists of a few seats $k_i = \{  k_{i(1,1)},  k_{i(1,2)}, ..., k_{i(2,1)},  k_{i(2,2)}, ...   \}$ where $k_{i(r,c)}$ denotes the seat in $r$-th row $c$-th column in block $k_i$. %\textcolor{blue}{Two days is set as the length of the time interval in our application.}

% Based upon block and time interval definition, we define a bin ${b}_{t_j}^{k_i}$ as a spatio-temporal conception which corresponds to block $k_i$ across the whole time interval $t_j$. $B_{t_j} = \{{b}_{t_j}^{k_1}, {b}_{t_j}^{k_2}, ..., {b}_{t_j}^{k_n}\}$ is the collection of all the bins at time interval $t_j$. 
% And  $p_{t_j}^{b_i}$ is the bin price of ${b}_{t_j}^{k_i}$, which is computed by the average of all the available selling prices in bin ${b}_{t_j}^{k_i}$.

% We name this conversion from seat prices to bin prices as ``coarsening". This coarsening layer is similar to average pooling layer in traditional CNN. However, there are two differences: 1)unlike pooling layer, it doesn't only compress spatial information but also temporal;  2) the motivation of pooling is to reduce the size and amount of parameters, but our coarsening layer is to reduce the spatio-temporal sparsity on the input data. 

% We further define $P_{t_j} = \{  p_{t_j}^{b_1}, p_{t_j}^{b_2}, ..., p_{t_j}^{b_n}\}$ as the bin prices of all the bins at time interval $t_j$. And we denote $p_{t_j}^{b_{i(r,c)}}$ as the ticket price of the seat in $r$-th row $c$-th column in bin $b_i$ at time $t_j$. Our first goal is to design a model $F$ to predict bin price:  
% \begin{align}
% \label{eq:goal}
% & P_{t_{j+1}} = F_1(P_{1},...P_{t_j}, C_{1},...C_{t_j}),  
% \end{align}  
% where $C_{t_j}$ are context features for the corresponding match at time interval $t_j$. 
% Furthermore, since it is important to predict each seat's selling price so that the campaign plan can be more oriented to specic groups of potential customers, we also want to predict the price of each seat:
% \begin{align}
% \label{eq:goal}
% & p_{t_{j+1}}^{b_{i(r,c)}} = F_2(P_{1},...P_{t_j}, C_{1},...C_{t_j}).  
% \end{align}  

% \subsection{Bin Size for Temporal Coarsening}
% Another complication of the temporal data is the uneven distribution of transaction times, or MTG (minutes till game). It is observed that ticket sales are rare when MTG is large, and number of transactions increase exponentially as MTG becomes smaller and closer to the game. Therefore, we used logarithm $log{MTG}$. Then, to mark $N$ bins, we start with largest $log{MTG}$ that contains 95\% of data, as $log{MTG}_{start}$. $log{MTG}_{end}$ is set to $0$. This is because even though ticket sales with MTG less than 1 happens very rarely. But when it happens, it would drive down $log{MTG}$ to negative infinity. So we simply excluded them from bin calculations first. $N$ bins are then calculated from $log{MTG}_{start}$ till $log{MTG}_{end}$ evenly. Then the leftover  data are added to their closest bins respectively.  

% %% https://www.quora.com/What-is-the-difference-between-Deconvolution-Upsampling-Unpooling-and-Convolutional-Sparse-Coding
% %% https://en.wikipedia.org/wiki/Bilevel_optimization

